A Fast Algorithm for Adaptive Private Mean Estimation

We design an $(\varepsilon, \delta)$-differentially private algorithm to estimate the mean of a $d$-variate distribution, with unknown covariance $\Sigma$, that is adaptive to $\Sigma$. To within polylogarithmic factors, the estimator achieves optimal rates of convergence with respect to the induced Mahalanobis norm $||\cdot||_\Sigma$, takes time $\tilde{O}(n d^2)$ to compute, has near linear sample complexity for sub-Gaussian distributions, allows $\Sigma$ to be degenerate or low rank, and adaptively extends beyond sub-Gaussianity. Prior to this work, other methods required exponential computation time or the superlinear scaling $n = \Omega(d^{3/2})$ to achieve non-trivial error with respect to the norm $||\cdot||_\Sigma$.

==> preamble.tex <==
% -*- mode: latex -*- %

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage{geometry}
\geometry{verbose,tmargin=1in,bmargin=1in,lmargin=3cm,rmargin=3cm}

\usepackage{babel}
\usepackage{array}
\usepackage{verbatim}
\usepackage{diagbox}
\usepackage{enumitem}
\usepackage{xifthen}

\usepackage{amsmath, amsfonts, amsthm, bm,  amssymb, longtable, multirow, mathrsfs}
% \usepackage{epstopdf, graphicx, subcaption, dsfont}
% \usepackage{algorithm}  
% \usepackage{algorithmicx}  
\usepackage{algpseudocode}
\usepackage{booktabs}
\usepackage{array}
\usepackage{booktabs}
\usepackage[numbers]{natbib}

\usepackage{setspace}
%% \onehalfspacing
% \usepackage{parskip}

\usepackage{xcolor}

\usepackage[ruled,linesnumbered,noend]{algorithm2e}

% \usepackage{cleveref}

\definecolor{darkblue}{rgb}{0,0,.5}
\RequirePackage[colorlinks,allcolors=darkblue]{hyperref}

\usepackage[capitalize]{cleveref}
\usepackage{crossreftools}

\allowdisplaybreaks

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}

\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}[section]
\newtheorem{claim}[lemma]{Claim}

\theoremstyle{definition}

\newtheorem{assumption}{Assumption}
\renewcommand{\theassumption}{A\arabic{assumption}}
\newtheorem{definition}{Definition}

\theoremstyle{remark}
\newtheorem*{rem}{Remark}
\newtheorem*{note}{Note}

\newcounter{example}
\newenvironment{example}[1][]{
  \refstepcounter{example}
  \ifthenelse{\isempty{#1}}{%
    % There is no text to display in the example
    \noindent \textbf{Example \theexample:}\hspace*{.05em}
  }{%
    \noindent \textbf{Example \theexample} ({#1})\textbf{:}\hspace*{.05em}
  }
}{%
  $\Diamond$ \medskip
}


\newenvironment{sproof}{\renewcommand{\proofname}{Proof sketch}\proof}{\endproof}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

\newlength{\phaserulewidth}
\newcommand{\setphaserulewidth}{\setlength{\phaserulewidth}}
\newcommand{\phase}[1]{
  %
  % Top phase rule
  \nonl\hrulefill\\
  \nonl\strut#1\\% Phase text
  % Bottom phase rule
  % \nonl\vspace{-1.25ex}\leavevmode\rule{\linewidth}{\phaserulewidth}\;
  \nonl\vspace{-1.25ex}\hrulefill\\
}
\setphaserulewidth{.7pt}

\usepackage{listings}
\usepackage{amssymb}

